A Labelled Sequent Calculus for BBI: Proof Theory and Proof Search

We present a labelled sequent calculus for Boolean BI, a classical variant of O'Hearn and Pym's logic of Bunched Implication. The calculus is simple, sound, complete, and enjoys cut-elimination. We show that all the structural rules in our proof system, including those rules that manipulate labels, can be localised around applications of certain logical rules, thereby localising the handling of these rules in proof search. Based on this, we demonstrate a free variable calculus that deals with the structural rules lazily in a constraint system. A heuristic method to solve the constraints is proposed in the end, with some experimental results.

==> proofsearch.tex <==
\section{Localising structural rules}
\label{sec:proofsearch}

In this section, we show that the applications of the structural rules of $\lsbbi$ can be
restricted so that they appear as clusters of rules around certain logical rules. 
This is proved by a permutation argument: we show that structural rules can be permuted 
upwards until the application of $\mand R$, $\mimp L$, $id$, or
$\top^* R$ is necessary. We refer to these four rules as
\textit{positive} rules, the rest of the logical rules are \textit{negative}
rules. We say a $\lsbbi$ derivation is \textit{strategic} if there is
no negative rule applications between any structural rule applications
and positive rule applications.

\begin{lemma}
\label{lem_abs_s1}
In $\lsbbi$, any derivation can be transformed into a strategic derivation.
\end{lemma}

\begin{proof}
To prove this lemma, we need to show that if a derivation involves the
structural rules, we can always apply them exactly before $\mand R$
and $\mimp L$, or before zero-premise rules. We show this by an
induction on the height of the derivation. Since we do not permute
structural rules through zero-premise rules, the proof in the base
case and the inductive step are essentially the same. Here we give
some examples of the permutations. Assuming the lemma holds up to any
derivation of height $n-1$, consider a derivation of height $n$.

\begin{enumerate}
\item Permute the application of $Eq_1$ or $Eq_2$ through
  non-zero-premise logical rules except for $\mand R$ and $\mimp
  L$. Here we give some examples, the rest are similar.
\begin{enumerate}
\item Permute $Eq_2$ through additive logical rules is trivial, this
  is exemplified by $\land L$, assuming the label of the principal formula
  is modified by the $Eq_2$ application. The original derivation is as follows.
\begin{center}
\alwaysNoLine
\AxiomC{$\Pi$}
\UnaryInfC{$(\epsilon,\epsilon\simp
  \epsilon);\Gamma[\epsilon/w];\epsilon:A;\epsilon:B \vdash
  \Delta[\epsilon/w]$}
\alwaysSingleLine
\RightLabel{$\land L$}
\UnaryInfC{$(\epsilon,\epsilon\simp
  \epsilon);\Gamma[\epsilon/w];\epsilon:A\land B \vdash
  \Delta[\epsilon/w]$}
\RightLabel{$Eq_2$}
\UnaryInfC{$(\epsilon,\epsilon\simp
 w);\Gamma;w:A\land B \vdash
  \Delta$}
\DisplayProof
\end{center}

The derivation is changed to the following:
\begin{center}
\alwaysNoLine
\AxiomC{$\Pi$}
\UnaryInfC{$(\epsilon,\epsilon\simp
  \epsilon);\Gamma[\epsilon/w];\epsilon:A;\epsilon:B \vdash
  \Delta[\epsilon/w]$}
\alwaysSingleLine
\RightLabel{$Eq_2$}
\UnaryInfC{$(\epsilon,\epsilon\simp
 w);\Gamma;w:A; w:B \vdash
  \Delta$}
\RightLabel{$\land L$}
\UnaryInfC{$(\epsilon,\epsilon\simp
 w);\Gamma;w:A\land B \vdash
  \Delta$}
\DisplayProof
\end{center}

\item Permute $Eq_1$ through $\top^* L$, assuming the label of
  principal formula is $w$. The derivation is as follows.
\begin{center}
\alwaysNoLine
\AxiomC{$\Pi$}
\UnaryInfC{$(\epsilon,\epsilon\simp
  \epsilon);\Gamma[w/w'][\epsilon/w]\vdash \Delta[w/w'][\epsilon/w]$}
\alwaysSingleLine
\RightLabel{$\top^* L$}
\UnaryInfC{$(\epsilon,w\simp
 w);\Gamma[w/w'];w:\top^*\vdash \Delta[w/w']$}
\RightLabel{$Eq_1$}
\UnaryInfC{$(\epsilon,w'\simp
 w);\Gamma;w':\top^*\vdash \Delta$}
\DisplayProof
\end{center}

We modify the derivation as follows.
\begin{center}
\alwaysNoLine
\AxiomC{$\Pi$}
\UnaryInfC{$(\epsilon,\epsilon\simp
  \epsilon);\Gamma[\epsilon/w'][\epsilon/w]\vdash \Delta[\epsilon/w'][\epsilon/w]$}
\alwaysSingleLine
\RightLabel{$Eq_2$}
\UnaryInfC{$(\epsilon,\epsilon\simp
 w);\Gamma[\epsilon/w']\vdash \Delta[\epsilon/w']$}
\RightLabel{$\top^* L$}
\UnaryInfC{$(\epsilon,w'\simp
 w);\Gamma;w':\top^*\vdash \Delta$}
\DisplayProof
\end{center}

Notice that the premises of the two derivations below $\Pi$ are
exactly the same. The application of $Eq_1$ in the original derivation
is changed to an application of $Eq_2$ in the modified derivation. However,
this does not break the proof, as the induction hypothesis ensures that
either of them can be permuted upwards.

Also, the label of principal formula in the rule $\top^* L$ cannot be
the one that is replaced in the rule $Eq_2$ below it, this is the
reason we do not exemplify this situation using $Eq_2$.

\item Permute $Eq_2$ through $\mand L$, assuming the label of
  principal formula is $z$, and it is modified by the $Eq_2$ application.
\begin{center}
\alwaysNoLine
\AxiomC{$\Pi$}
\UnaryInfC{$(x,y\simp \epsilon);(\epsilon,\epsilon\simp \epsilon);\Gamma[\epsilon/z];x:A;y:B\vdash
  \Delta[\epsilon/z]$}
\alwaysSingleLine
\RightLabel{$\mand L$}
\UnaryInfC{$(\epsilon,\epsilon\simp \epsilon);\Gamma[\epsilon/z];\epsilon:A\mand B\vdash
  \Delta[\epsilon/z]$}
\RightLabel{$Eq_2$}
\UnaryInfC{$(\epsilon,\epsilon\simp z);\Gamma;z:A\mand B \vdash \Delta$}
\DisplayProof
\end{center}

Since $x$ and $y$ are fresh labels, they will not be affected by
$Eq_2$. Thus the derivation can be changed to the following:
\begin{center}
\alwaysNoLine
\AxiomC{$\Pi$}
\UnaryInfC{$(x,y\simp \epsilon);(\epsilon,\epsilon\simp \epsilon);\Gamma[\epsilon/z];x:A;y:B\vdash
  \Delta[\epsilon/z]$}
\alwaysSingleLine
\RightLabel{$Eq_2$}
\UnaryInfC{$(x,y\simp z);(\epsilon,\epsilon\simp z);\Gamma;x:A;y:B\vdash
  \Delta$}
\RightLabel{$\mand L$}
\UnaryInfC{$(\epsilon,\epsilon\simp y);\Gamma;z:A\mand B \vdash \Delta$}
\DisplayProof
\end{center}

Since $Eq_1$ and $Eq_2$ only globally replaces labels, their
action can be safely delayed through all the rules other than $\mand R$ and $\mimp L$. The applications of these two rules after the last $\mand R$ or $\mand L$ will be delayed until the zero-premise rule is necessary.
\end{enumerate}

\item Permute the applications of $E$, $U$, $A$, and $A_C$ through non-zero premise logical rules other than $\mand R$ and $\mimp L$. Again, we give some examples, the rest are similar.
\begin{enumerate} 
\item Permute $E$ through $\top^* L$, assuming the label of the principal
  formula is $y$.
The original derivation runs as follows.
\begin{center}
\alwaysNoLine
\AxiomC{$\Pi$}
\UnaryInfC{$(\epsilon,x\simp z);(x,\epsilon\simp z);\Gamma[\epsilon/y]
  \vdash \Delta[\epsilon/y]$}
\alwaysSingleLine
\RightLabel{$\top^* L$}
\UnaryInfC{$(y,x\simp z);(x,y\simp z);\Gamma;y:\top^*
  \vdash \Delta$}
\RightLabel{$E$}
\UnaryInfC{$(x,y\simp z);\Gamma;y:\top^*
  \vdash \Delta$}
\DisplayProof
\end{center}

The new derivation is as follows.
\begin{center}
\alwaysNoLine
\AxiomC{$\Pi$}
\UnaryInfC{$(\epsilon,x\simp z);(x,\epsilon\simp z);\Gamma[\epsilon/y]
  \vdash \Delta[\epsilon/y]$}
\alwaysSingleLine
\RightLabel{$E$}
\UnaryInfC{$(x,\epsilon\simp z);\Gamma[\epsilon/y]
  \vdash \Delta[\epsilon/y]$}
\RightLabel{$\top^* L$}
\UnaryInfC{$(x,y\simp z);\Gamma;y:\top^*
  \vdash \Delta$}
\DisplayProof
\end{center}

This shows that if the logical rule only does substitution, delaying
the application of structural rules makes no difference.

\item Permute $U$ through $\mand L$, assuming the label of the principal
  formula is $z$. The original derivation is as follows.
\begin{center}
\alwaysNoLine
\AxiomC{$\Pi$}
\UnaryInfC{$(x,y\simp z);(z,\epsilon\simp z);\Gamma;x:A;y:B \vdash
  \Delta$}
\alwaysSingleLine
\RightLabel{$\mand L$}
\UnaryInfC{$(z,\epsilon\simp z);\Gamma;z:A\mand B \vdash
  \Delta$}
\RightLabel{$U$}
\UnaryInfC{$\Gamma;z:A\mand B \vdash
  \Delta$}
\DisplayProof
\end{center}

The new derivation is as follows.
\begin{center}
\alwaysNoLine
\AxiomC{$\Pi$}
\UnaryInfC{$(z,\epsilon\simp z);(x,y\simp z);\Gamma;x:A;y:B \vdash
  \Delta$}
\alwaysSingleLine
\RightLabel{$U$}
\UnaryInfC{$(x,y\simp z);\Gamma;z:A\mand B \vdash
  \Delta$}
\RightLabel{$\mand L$}
\UnaryInfC{$\Gamma;z:A\mand B \vdash
  \Delta$}
\DisplayProof
\end{center}

Since the labels $x$ and $y$ are all fresh labels, it is safe to
change the order to rule applications as above.

Additive logical rules are totally independent on the relational
atoms, so those cases are similar as the one shown above, except that
those rules do not add relational atoms to the sequent.

\end{enumerate}
\end{enumerate}
\end{proof}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

